Improving In-context Learning of Multilingual Generative Language Models with Cross-lingual Alignment

Multilingual generative models obtain remarkable cross-lingual in-context learning capabilities through pre-training on large-scale corpora. However, they still exhibit a performance bias toward high-resource languages and learn isolated distributions of multilingual sentence representations, which may hinder knowledge transfer across languages. To bridge this gap, we propose a simple yet effective cross-lingual alignment framework exploiting pairs of translation sentences. It aligns the internal sentence representations across different languages via multilingual contrastive learning and aligns outputs by following cross-lingual instructions in the target language. Experimental results show that even with less than 0.1 {\textperthousand} of pre-training tokens, our alignment framework significantly boosts the cross-lingual abilities of generative language models and mitigates the performance gap. Further analyses reveal that it results in a better internal multilingual representation distribution of multilingual models.

==> tabs/ablation/bloom_560m.tex <==
\begin{table}[th]
        \setlength{\tabcolsep}{3mm}
	\centering
	\scriptsize
	%\vspace{-0.4cm}
	\renewcommand\arraystretch{1.2}
	\begin{center}
		\begin{tabular}{lccc}
			\toprule[1.2pt]  
			\multicolumn{1}{c}{\textbf{Model}}                & \textbf{0-shot}              &  \textbf{3-shot}              &  \textbf{5-shot} \\
			\midrule[0.8pt]
			\multicolumn{1}{l}{$\text{BLOOM}_{\text{560M}}$}  & $51.91_{\pm 0.43}$           & $52.63_{\pm 0.51}$            & $52.57_{\pm 0.53}$\\
                \midrule[0.8pt]
                {\scriptsize w/ MCL}                              & $52.68_{\pm 0.34}$           & $52.01_{\pm 0.43}$            & $51.67_{\pm 0.55}$\\
                % {\scriptsize w/ CLM}                              & $53.22_{\pm 0.52}$           & $53.35_{\pm 0.52}$            & $53.43_{\pm 0.57}$\\
                {\scriptsize w/ MIT}                              & $53.45_{\pm 0.53}$           & $53.27_{\pm 0.56}$            & $53.58_{\pm 0.64}$\\
                {\scriptsize w/ CIT}                              & $54.71_{\pm 0.43}$           & $54.02_{\pm 0.47}$            & $54.13_{\pm 0.46}$\\
			{\scriptsize w/ AFP}                              & $\textbf{55.94}_{\pm 0.21}$  & $\textbf{55.04}_{\pm 0.32}$   & $\textbf{55.70}_{\pm 0.31}$\\
			\bottomrule[1.2pt]
		\end{tabular}
            \caption{\label{tab:ablation_study_bloom_560m}Ablation study of different training methods on 5 datasets for $\text{BLOOM}_{\text{560M}}$.}
	\end{center}
	% \vspace{-5mm}
\end{table}

==> tabs/generation/en_zh.tex <==
\begin{table*}[htp]

\renewcommand\arraystretch{1.3}

\centering
\scriptsize

\setlength{\tabcolsep}{0.6mm}

\caption{\label{tab:2lang_gen} In-context learning generation results on bilingual condition. 
}

 \begin{tabu}{lcccc}
 
 \toprule[1.2pt]
   & \multicolumn{2}{c}{\textbf{FLORES-101 (1/3/5)}} & \multicolumn{2}{c}{\textbf{Summarization (1/3)}} \\
  \cmidrule(r){2-3}  \cmidrule(r){4-5} \noalign{\smallskip}
\multicolumn{1}{c}{\textbf{Model}}& \textbf{EN$\to$ZH}&\textbf{ZH$\to$EN}& \textbf{EN$\to$ZH}&\textbf{ZH$\to$EN} \\

   \midrule[0.8pt]
 
  $\text{XGLM-564M}$               & $0.5/3.9/4.2$                              & $7.7/8.1/8.3$                                 & $0.1/0.3$                      & $0.4/0.5$                  \\
  
 \ \ \ \ \ \ \ \ \ +AFP            & $\textbf{4.2}/\textbf{5.3}/\textbf{5.9}$   & $\textbf{8.7}/\textbf{9.0}/\textbf{9.2}$      & $\textbf{0.5}/\textbf{0.4}$    & $\textbf{0.6}/\textbf{0.6}$   \\

 $\text{XGLM-1.7B}$                & $4.9/5.6/5.9$                              & $11.6/11.4/11.2$                              & $\textbf{40.9}/37.6$           & $40.0/38.1$                   \\
  
 \ \ \ \ \ \ \ \ \ +AFP            & $\textbf{6.6}/\textbf{7.2}/\textbf{8.4}$   & $\textbf{11.7}/\textbf{11.5}/\textbf{11.9}$   & $40.3/\textbf{44.0}$           & $\textbf{40.5}/\textbf{41.8}$ \\

 $\text{XGLM-7.5B}$                & $13.6/13.8/13.9$                           & $20.2/20.5/20.1$                              & $\textbf{40.9}/37.6$           & $40.0/38.1$                   \\
  
 \ \ \ \ \ \ \ \ \ +AFP            & $\textbf{15.5}/\textbf{15.8}/\textbf{16.0}$                                 & $\textbf{20.5}/\textbf{20.6}/\textbf{20.3}$                                   & $40.3/\textbf{44.0}$           & $\textbf{40.5}/\textbf{41.8}$ \\
 
 \specialrule{0em}{0pt}{0pt}

    % \cdashlinelr{1-9}
  \midrule[0.8pt]
  
$\text{BLOOM-560M}$                  & $44.4/40.4$                      & $41.1/40.3$                       & $33.4/35.1$                   & $34.5/34.1$                  \\
  
 \ \ \ \ \ \ \ \ \ +AFP              & $\textbf{51.4}/\textbf{47.5}$    & $\textbf{49.4}/\textbf{45.1}$     & $\textbf{38.8}/\textbf{40.5}$ & $\textbf{39.7}/\textbf{39.4}$ \\

$\text{BLOOM-1.7B}$                  & $50.4/44.4$                      & $47.6/46.1$                       & $37.9/35.7$                   & $36.9/35.0$                   \\

 \ \ \ \ \ \ \ \ \ +AFP              & $\textbf{53.0}/\textbf{51.3}$    & $\textbf{49.9}/\textbf{47.1}$     & $\textbf{41.2}/\textbf{41.8}$ & $\textbf{40.1}/\textbf{41.3}$ \\
 
 \specialrule{0em}{0pt}{0pt}


    
\bottomrule[1.2pt]
\end{tabu}

% \vspace{-2mm}

\end{table*}

==> tabs/generation/en_zh_translation.tex <==
\begin{table*}[ht]

\renewcommand\arraystretch{1.1}

\centering
\scriptsize

\setlength{\tabcolsep}{1.6mm}

 \begin{tabu}{l|cccc|cccc|cccc}
 
 \toprule[1.2pt]
  \multicolumn{1}{c}{\textbf{ }} & \multicolumn{4}{c}{\textbf{EN$\to$ZH}} & \multicolumn{4}{c}{\textbf{ZH$\to$EN}} & \multicolumn{4}{c}{\textbf{Avg}} \\
  \cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13}  \noalign{\smallskip}
\multicolumn{1}{c}{\textbf{Model}}& 0 & 1 & 5 & \multicolumn{1}{c}{10} & 0 & 1 & 5 & \multicolumn{1}{c}{10} & 0 & 1 & 5 &10 \\

   \midrule[0.8pt]
 
  $\text{XGLM}_{\text{564M}}$               & $0.0$&$1.0_{\pm 0.4}$&$4.2_{\pm 0.5}$&$4.2_{\pm 0.5}$                                       & $0.0$&$6.4_{\pm 0.6}$&$8.1_{\pm 0.4}$&$8.3_{\pm 0.5}$                                        & $0.0$&$3.7_{\pm 0.5}$&$6.0_{\pm 0.4}$&$6.3_{\pm 0.4}$   \\
  
 \ \ \ \ \ \ \ \ \ +AFP            &$\textbf{2.0}$&$\textbf{4.2}_{\pm 0.3}$&$\textbf{5.3}_{\pm 0.3}$&$\textbf{5.9}_{\pm 0.2}$    &$\textbf{5.3}$&$\textbf{8.7}_{\pm 0.6}$&$\textbf{9.0}_{\pm 0.5}$&$\textbf{9.2}_{\pm 0.4}$     & $\textbf{3.7}$&$\textbf{6.5}_{\pm 0.5}$&$\textbf{7.2}_{\pm 0.3}$&$\textbf{7.6}_{\pm 0.3}$   \\
 
    \cdashlinelr{1-13}

 $\text{XGLM}_{\text{7.5B}}$       &$0.0$ & $13.6_{\pm 1.1}$&$13.8_{\pm 0.9}$&$13.9_{\pm 0.7}$     & $0.1$&$19.2_{\pm 0.7}$&$19.5_{\pm 0.8}$&$20.1_{\pm 0.4}$       & $0.1$&$16.4_{\pm 0.8}$&$16.7_{\pm 0.6}$&$17.0_{\pm 0.4}$ \\
  
 \ \ \ \ \ \ \ \ \ +AFP            &$\textbf{2.5}$&$\textbf{14.5}_{\pm 0.8}$&$\textbf{14.8}_{\pm 0.6}$&$\textbf{15.0}_{\pm 0.6}$ &$\textbf{6.7}$& $\textbf{19.5}_{\pm 0.6}$&$\textbf{19.6}_{\pm 0.5}$&$\textbf{20.3}_{\pm 0.3}$ & $\textbf{4.6}$&$\textbf{17.0}_{\pm 0.6}$&$\textbf{17.2}_{\pm 0.5}$&$\textbf{17.7}_{\pm 0.4}$    \\
 %  \midrule[0.8pt]

 %   $\text{BLOOM}_{\text{560M}}$             & $0.1$&$1.5$&$2.8$&$3.2$                                       & $0.2$&$1.8$&$3.3$&$3.5$                                        & $0.2$&$1.7$&$3.1$&$3.2$    \\
  
 % \ \ \ \ \ \ \ \ \ +AFP            & $\textbf{1.5}$&$\textbf{3.1}$&$\textbf{4.0}$&$\textbf{4.5}$   & $\textbf{2.2}$&$\textbf{3.6}$&$\textbf{4.3}$&$\textbf{4.9}$    & $\textbf{1.9}$&$\textbf{3.4}$&$\textbf{4.2}$&$\textbf{4.7}$    \\
 
 %    \cdashlinelr{1-13}

 % $\text{BLOOM}_{\text{7.1B}}$               & $2.0$&$8.1$&$8.2$&$9.7$                                       & $3.0$&$10.6$&$12.0$&$12.4$                                     & $2.5$&$9.3$&$10.2$&$11.1$   \\
  
 % \ \ \ \ \ \ \ \ \ +AFP            & $\textbf{4.5}$&$\textbf{9.8}$&$\textbf{10.2}$&$\textbf{10.5}$ & $\textbf{5.1}$&$\textbf{11.0}$&$\textbf{12.4}$&$\textbf{12.7}$ & $\textbf{4.8}$&$\textbf{10.4}$&$\textbf{11.3}$&$\textbf{11.6}$  \\
 
 % \specialrule{0em}{0pt}{0pt}


    
\bottomrule[1.2pt]
\end{tabu}

\vspace{-2mm}
\caption{\label{tab:2lang_gen} Translation results on FLORES-101 devtest set. 
}

\vspace{-4mm}

\end{table*}

==> tabs/llama_aug/zh_en.tex <==
\begin{table*}[htp]

\renewcommand\arraystretch{1.3}

\centering
\scriptsize

\setlength{\tabcolsep}{0.3mm}

\caption{\label{tab:zh_en_llama} In-context learning results of LLaMA on 5 datasets. 
}

 \begin{tabu}{lcccccccccc}
 
 \toprule[1.2pt]
   & \multicolumn{2}{c}{\textbf{XNLI}} & \multicolumn{2}{c}{\textbf{PAWS-X}} & \multicolumn{2}{c}{\textbf{XCOPA}} & \multicolumn{2}{c}{\textbf{XStoryCloze}} & \multicolumn{2}{c}{\textbf{XWinograd}} \\
  \cmidrule(r){2-3}  \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \noalign{\smallskip}
\multicolumn{1}{c}{\textbf{Model}}& \textbf{EN-0/5}&\textbf{ZH-0/5}& \textbf{EN-0/5}&\textbf{ZH-0/5}& \textbf{EN-0/5}&\textbf{ZH-0/5}& \textbf{EN-0/5}&\textbf{ZH-0/5} & \textbf{EN-0/5}&\textbf{ZH-0/5} \\

   \midrule[0.8pt]
 
  $\text{Alpaca-7B}$                  & $45.5/42.9$                      & $39.0/39.3$                       & $51.0/52.4$                   & $50.9/48.8$                   & $62.4/64.0$                   & $56.4/57.8$                   & $62.7/64.5$   & $56.3/56.3$   & $57.2/60.0$   & $68.3/\textbf{69.6}$\\
 
  $\text{ChineseAlpaca-7b}$                  & $47.6/38.2$                      & $37.6/35.6$                       & $50.4/46.6$                   & $52.6/48.8$                   & $56.4/59.6$                   & $52.8/52.2$                   & $59.6/60.8$   & $54.3/52.9$   & $54.8/56.7$   & $\textbf{67.5}/\textbf{67.3}$\\

  $\text{LLaMA-7B}$                  & $54.1/49.9$                      & $45.4/44.2$                       & $58.9/56.3$                   & $51.1/55.8$                   & $69.4/74.6$                   & $\textbf{64.4}/63.2$                   & $69.2/73.7$   & $59.5/59.2$   & $62.8/66.4$   & $73.8/\textbf{74.0}$\\
 \ \ \ \ \ \ \ \ \ +MIL            & $\textbf{55.0}/\textbf{56.0}$    & $\textbf{48.0}/\textbf{48.8}$       & $\textbf{64.8}/\textbf{61.2}$ & $\textbf{57.8}/\textbf{56.4}$  & $\textbf{72.2}/\textbf{75.6}$ & $64.2/\textbf{66.8}$  & $\textbf{72.0}/\textbf{74.7}$   & $\textbf{62.7}/\textbf{63.4}$   & $\textbf{65.2}/\textbf{68.2}$   & $\textbf{75.8}/73.2$\\
 
 \ \ \ \ \ \ \ \ \ +AFP(ours)            & $\textbf{55.0}/\textbf{56.0}$    & $\textbf{48.0}/\textbf{48.8}$       & $\textbf{64.8}/\textbf{61.2}$ & $\textbf{57.8}/\textbf{56.4}$  & $\textbf{72.2}/\textbf{75.6}$ & $64.2/\textbf{66.8}$  & $\textbf{72.0}/\textbf{74.7}$   & $\textbf{62.7}/\textbf{63.4}$   & $\textbf{65.2}/\textbf{68.2}$   & $\textbf{75.8}/73.2$\\
 
 \specialrule{0em}{0pt}{0pt}


    
\bottomrule[1.2pt]
\end{tabu}

% \vspace{-2mm}

\end{table*}
